Embedding Session Types in HML

Recent work on the enhancement of multiparty session types with logical annotations enable the effective verification of properties on (1) the structure of the conversations, (2) the sorts of the messages, and (3) the actual values exchanged. In [3] we extend this work to enable the specification and verification of mutual effects of multiple cross-session interactions. Here we give a sound and complete embedding into the Hennessy-Milner logic to justify the expressiveness of the approach in [3] and to provide it with a logical background that will enable us to compare it with similar approaches.

==> eptcsdata.tex <==
\providecommand{\firstpage}{53}
\providecommand{\publicationstatus}{N. Yoshida, W. Vanderbauwhede (Eds.): Programming Language\\ Approaches to Concurrency- and Communication-cEntric\\Software 2013 (PLACES'13)\\
EPTCS 137, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.137.5}{10.4204/EPTCS.137.5}}

